Characterizing Barriers and Technology Needs in the Kitchen for Blind and Low Vision People

Cooking is a vital yet challenging activity for people with visual impairments (PVI). It involves tasks that can be dangerous or difficult without vision, such as handling a knife or adding a suitable amount of salt. A better understanding of these challenges can inform the design of technologies that mitigate safety hazards and improve the quality of the lives of PVI. Furthermore, there is a need to understand the effects of different visual abilities, including low vision and blindness, and the role of rehabilitation training where PVI learn cooking skills and assistive technologies. In this paper, we aim to comprehensively characterize PVI's challenges, strategies, and needs in the kitchen from the perspectives of both PVI and rehabilitation professionals. Through a contextual inquiry study, we observed 10 PVI, including six low vision and four blind participants, when they cooked dishes of their choices in their own kitchens. We then interviewed six rehabilitation professionals to explore their training strategies and technology recommendations. Our findings revealed the differences between low vision and blind people during cooking as well as the gaps between training and reality. We suggest improvements for rehabilitation training and distill design considerations for future assistive technology in the kitchen.

==> Sections/5-Discussion.tex <==
\section{Discussion}
%Summary of our resarch - two studies; emphasize our contribution, uniqueness, and key finding
%connection between study 1 and study 2
    %tools recommended in the training were not used in real life (e.g., palm peeler); technology awareness 
    %professionals' limited exposure of latest tech
%Challenges remained even after training:
%1. find things ad hoc
%2. get burnt even wearing mitts or gloves
%Technology implications
%1. remote communication tool to support small group training? - VR?
%2. technology to support interaction with appliance interfaces. Guo's research. However, need to hold the smartphone, hands-free device? smartglasses? Screen reader embedded into appliance interfaces - more burden on manufacture 
%3. tech to deal with hot elements. 
%4. tech for cutting? recognize blade position and highlight?
%5. tech for low vision, especially who has recent vision loss
%low tech vs high tech - needs technology that is easy to learn, social acceptable, and intelligent - smart speaker is widely accepted. low cost is important. benefits of high tech - e.g., smartspeaker
%technology for people with low vision/recent vision loss
%technology for safety
%VR training 
Our research contributed a thorough observation of PVI's cooking experience as well as the first investigation on the rehabilitation training process for kitchen activities. Unlike prior works that focused on interviews \cite{kashyap2020behaviors, li2021non} and YouTube video observations \cite{li2021non}, we conducted a contextual inquiry study with 10 PVI (six low vision and four blind) to achieve first-hand observations. Beyond confirming major findings from prior work, our observation also revealed details that would not be easily uncovered with other study methods. For example, %participants used a replacement (e.g., a back scratcher) of a white cane to navigate a small and crowded kitchen, and 
while keeping things organized in the kitchen, participants still lost track of things during the dynamic and busy cooking process;
while wearing protective gloves, participants still got their arms burnt when using an oven. Moreover, our study involved both blind and low vision participants, highlighting their different challenges, strategies, and needs in doing cooking tasks. 

%This study highlighted differences between blind people and low vision people regarding their cooking experience, needs, and perspectives on technology, where people with low vision were generally less confident working in the kitchen. 

Understanding the rehabilitation training process for cooking was another important aspect of our research. We interviewed six rehabilitation professionals from different programs and observed some training sessions. This study revealed the detailed training process, principles followed by the professionals, specific training content and skills, and limitations of current training. While different services offered different training plans, we found that most professionals provided the flexibility to customize the training procedure based on PVI's abilities and needs. 
%For example, they taught touching strategies to blind clients, while emphasizing vision use for low vision clients. 

The two studies with PVI and rehabilitation professionals enabled us to develop a comprehensive understanding of PVI's experience and needs in the kitchen. We discussed how rehabilitation training may affect PVI's cooking experience, the difference between blind and low vision people in the kitchen context, and the design considerations for future kitchen technology for PVI by drawing insights from both studies. 

%Moreover, since we also asked about PVI’s training experience and how it helped them work in the kitchen, we became interested in trainers’ experience with providing cooking lessons for PVI. Thus, our research of interviewing trainers and observing training sessions contributed to the first exploration of what cooking training looked like for PVI as well as how the training was conducted. From both observations of PVI and in-depth interviews with trainers, we identified common challenges in the kitchen, including safety concerns (i.e., cutting and heat), measuring, transferring, and checking the doneness of food \cite{li2021non}. Additionally, based on these challenges and PVI's and trainers' preferences, we formulated ideas below of designing technology to make it more suitable and relevant for PVI.

%observing PVI cooking in the kitchen allowed us to have a comprehensive picture of how they navigated in the kitchen, including their movement, difficulties they faced, tools they used, and the overall setup of their kitchens. 
 
\subsection{Rehabilitation Training and Cooking in Real Life}
Little research had investigated the rehabilitation training process and its impact on PVI via the lens of HCI. Our research explored the training process and strategies in different rehabilitation programs (Study 2) as well as how the training experience affected PVI's cooking in real life (Study 1). We discussed the impact, limitations, and potential improvements of rehabilitation training from different aspects below.

\textbf{\textit{Effectiveness of Training.}} Rehabilitation training is helpful and can largely affect PVI's cooking habits. In our study with PVI (Study 1), we observed that participants used a lot of cooking skills and tools they learned from their rehabilitation training. For example, Derek spoke highly of the George Forman Grill recommended by his occupational therapist and used it frequently. Moreover, the cooking tasks in the training were all major challenges mentioned by our visually impaired participants in Study 1. We also found a big overlap between the cooking strategies and tools introduced by the professionals (Study 2, Section \ref{training content}) and the actual strategies used by PVI during cooking (Study 1) across all cooking tasks. The consistent results between the two studies indicated the effectiveness and practicality of the training to be applied to real-world cooking. 

\textbf{\textit{Generalizability.}} While the training provides useful strategies and tools, the skills learned from the training may not be easily transferred to PVI's real-life since their actual kitchen environments are usually more complex and challenging than the ideal training environments. Thus, both the professionals (e.g., Rachel) and PVIs (e.g., Mary) emphasized the importance of practicing at home, although some professionals were concerned about practicing without supervision could bring safety risks at the early stage of training. In the future, researchers should consider how to foster the generalizability of rehabilitation training to PVI's personal kitchen environments. For example, virtual reality-based training could be leveraged to simulate different kitchen environments to help PVI adapt to complex real-life kitchen situations more quickly, as well as providing PVI more practice opportunities without putting them at risk. 

\textbf{\textit{Group training.}} Compared to one-on-one training, group training provided PVI opportunities to communicate and learn from others (Study 1) and improved the training efficiency by training multiple clients at once (Study 2). However, according to the rehabilitation professionals, such a training format was harder to manage given the different needs and learning abilities of different clients. Moreover, the group training was more susceptible to external factors, and for example, many group sessions were suspended due to the COVID-19 pandemic. Thus, it is important to consider how to facilitate the management and customized training in a group setting. 
For example, collaborative technologies could help PVI and professionals schedule and coordinate group sessions. Personalized devices could also be used as a complementary tool in the group training session to help monitor the progress of each client and keep the professionals updated. Systems that fulfill such purposes have been explored in the field of educational technology \cite{silva2014glassist, holstein2019co}. There is a potential to apply and adapt these systems to the rehabilitation training context for PVI. 
Moreover, VR-based training can potentially remove the social barriers brought by the pandemic. 


\textbf{\textit{Access to Training and Technology Resources.}} %Our research also revealed the limitations of the current training from both PVI and the professionals' perspective. 
Both PVI and professional trainers indicated limited access to resources. In Study 1, several PVI mentioned that they did not know how to get rehabilitation training and whether they were eligible for it. Even participants with training experience reported the difficulty of gaining sufficient training due to the limited resource in the training program (e.g., Dixie). Also, in terms of technology, many advanced assistive devices were expensive and not covered by insurance, which may not be affordable to many PVI. This resource limitation was also reflected by the rehabilitation professionals. For example, many professionals mentioned not having enough time and resources to keep updated to new technologies, so their technology recommendations usually focused on low-tech tools. Moreover, for students with visual impairments, their training (i.e., IEP) had to make way for the general academic curriculum, which further limited their time for training on living skills. Unfortunately, the resource and time limitations could not be simply addressed by technology. More stakeholders in this field should be involved, from the clients and professionals to the rehabilitation service or organizations, the insurance companies, and the government.    

%It is important to consider how to address the time and resource limitation from both 

%limited resource to access, need more sessions; but professionals are limited and busy; 

%\textbf{\textit{Generalizability of Training Skills.}}
%not cover all challenges;
%sometimes hard to be applied 
%takes time to practice and adapt

%\textbf{\textit{Directions of Improvements.}}


%Trainings are helpful; many people used the strategies that they learnt from training; however, training was not sufficient; cannot learn everything - agreed by both PVI and OTs; also training cannot fully compensate for the vision loss that people acquired later in their life, at least not within short period. needs time to adapt. 

%improvement for Rehabilitation
%    VR simulation
%    Emotion control? 
%    improvement for tech exposure

\subsection{Blindness vs. Low Vision in the Kitchen Context}
Our research comprehensively investigated the cooking experiences of both blind and low vision people and uncovered their major differences in cooking activities. Our research showed that low vision participants, in general, were less confident and felt less safe than blind people in the kitchen (Figure \ref{fig:blv_likert}).
Instead of relying on audio and tactile cues, low vision people looked for and even purposely created visual cues (e.g., color contrast, size contrast, reflections) to leverage their residual vision in the kitchen. For example, they shook the pan and observed the motion of the egg to check its doneness (e.g., Jacob), and used cutting boards with different colors as opposed to the background to generate contrast (e.g., Derek). The rehabilitation professionals also distinguished blind and low vision clients when planning training content, encouraging low vision clients to make the most of their residual vision in cooking. Moreover, low vision participants leveraged vision enhancement technology in the kitchen, such as optical or digital magnifiers. However, these technologies only helped with the basic reading task (e.g., reading food packages and recipes) and could not fully support low vision people's needs in other cooking tasks, such as distinguishing hot elements, cutting, and navigating the crowded kitchen safely (e.g., Rachel).

%for example, it was not safe to use magnification when navigating the crowded kitchen. 

While myriad research had explored the challenges and needs of blind people and designed technology for them, little research had focused on the unique needs of low vision people. Recently, low vision research has attracted more attention with researchers exploring visual augmentations for low vision people in different tasks, including visual search and navigation \cite{zhao2016cuesee, zhao2020effectiveness}. No research has looked into cooking tasks. It is unknown whether existing visual augmentations could be applied in the crowded and busy kitchen context. Future research should consider low vision people's specific needs and design technologies to assist them in the kitchen context by generating visual cues, for example recognizing sharp tools in the kitchen and generating highlights via smart glasses. 

\subsection{Technology Design Considerations for PVI in the Kitchen.}
Combining PVI's needs and the rehabilitation professionals' suggestions in our studies, we distill design considerations for technology that facilities cooking tasks for PVI. 
%\subsection{The Lack of Technology Awareness.}

%\subsubsection{General Preferences.} From both Study 1 and Study 2, we found that PVI had an overall preference for low-tech tools over high technology. They owned and used more low-tech tools and expressed more positive attitude toward low-tech tools than high technology. On top of that, neither participants in Study 1 or trainers in Study 2 had much experience with high technology products, and both of them reported drawbacks of high technology that made it harder for them to use high technology.

%\subsubsection{Low-tech Tools Gap.}
%Despite  PVI’s preference for low-tech tools in Study 1 as well as clients’ positive feedback on those tools in Study 2, we did not observe any participant in Study 1 using those tools recommended by trainers. For example, during an observation session led by Rachel, she recommended her client to use a palm peeler instead of a handheld peeler, and upon the client learning and using the palm peeler, they found it very helpful as it significantly lowered the risk of getting cut. Along with other low-tech tools mentioned in the training and interviews, we did not identify any tools used by PVI that overlapped with trainers’ recommendations. We deduced that there was a gap between what PVI used and what trainers recommended, and PVI were not aware of tools used in the training. Thus, we proposed that on the one hand, resources, such as seminars, could be helpful to introduce PVI to learn about more diverse tools, and on the other hand, companies or organizations that manufactured these tools could make their products more visible through propagation or advertisement.

%\subsubsection{Insufficient Experience with High Technology.}
%As for high technology, in both studies, we found that both PVI and trainers did not have much experience with advanced technology (e.g.,) and did not prefer to use it. They reported that some features of advanced technology made it inaccessible to them. For example, advanced technology often came with flat screens that were hard to navigate as PVI preferred knobs or dials that gave them tactile feedback. Also, high costs and learning curves were also factors that made advanced technology less favorable. On top of that, the general lack of experience with advanced technology could also contribute to this phenomenon. Even for trainers, only two of them (Rachel and Lyla) had relatively more experience with advanced technology. As a result, PVI and trainers might only know a few technology products and were not aware of other options with more various and potentially, more accessible designs. Therefore, we believed that education on technology could be helpful to present more diverse options to PVI along with information and instruction on how to use it.


\subsubsection{Technology to Facilitate Safe Cooking.}
Kitchen safety is a critical issue emphasized by both PVI and rehabilitation professionals. The biggest safety concerns reported in both studies were cutting and interacting with heat \cite{kashyap2020behaviors,li2021non}. Participants reported several cases of getting injured in the kitchen, such as cutting themselves when using a grater (David) or burning their hands when moving the pot on the burner (Judy). Thus, it is vital to design technologies to guarantee PVI's safety in the kitchen. For example, a smart stove connects to the user's smartphone to inform the current temperature of each burner, or an AI-based system recognizes the exact position of knife blades and hot area and generates augmentations or alerts to PVI when their hands are close to the dangerous area (e.g., visual augmentation for low vision people, and audio warnings for blind people). Since touching was encouraged by the rehabilitation professionals (e.g., Maria), an intelligent guidance system that safely guides the PVI's hands during cooking could also be helpful. 

%To start with cutting, PVI often worried about getting injured, and thus, we proposed that smart cutting tools that could distinguish inanimate objects (i.e., food) from human hands could help prevent cutting injuries. Moreover, many PVI complained that it was hard for them to cut uniform pieces which could impact the doneness of food. Therefore, it would be helpful to have technology that could detect sizes of food pieces and help PVI cut uniformly. As for interacting with heat or hot surfaces, we proposed that having warning signs, visual, auditory, or both, could help prevent burns. For example, after using burners, the stove could not only have a visual indication if the burner was still hot but also connect to PVI’s phone or home system to let them know when it was hot or cold through audio or auditory cues. On top of that, we also thought that it would be helpful if PVI’s devices, such as smart glasses or even smart gloves, could warn them of the high temperature if they were near the heat source, especially under circumstances that PVI was not aware of a nearby heat source.

\subsubsection{Hands-free Interactions.}
Hands-free technology was suggested by both PVI and the professionals so that PVI could use both hands for cooking activities. For example, some low vision participants mentioned the difficulty of using a handheld magnifier when cutting (Chloe). Thus, instead of smartphone applications \cite{guo2016vizlens, guo2019statelens}, hands-free interactions are necessary for assistive technology in the kitchen. Both wearable devices (e.g., smart glasses, smartwatches) \cite{lang2021pressing} and IoT devices that are embedded in the kitchen \cite{sato2014shadow} could be considered to facilitate the need to use both hands. %While some hands-free systems have been designed to enhance cooking activities, for example, an projector-based augmented reality system that embeds into the kitchen to recognize the kitchen object on a kitchen counter and project visual instructions to guide a user through the cooking process  . 

%Specifically, wearable technology, such as smartwatches, smart glasses, and devices that could be worn around the chest, would be helpful when they were combined with, for example, cameras as they could help PVI use both hands to identify items they were looking for more efficiently and accurately \cite{lang2021pressing}. Another way to implement the hands-free feature was allowing devices to be fixed to the desired location would also be helpful since PVI would not have to take the device with them. For example, people with residual vision could have lighting devices fixed to walls of the storage room for easier identification or fixed to a desktop where they might access food recipes. In this way, they would neither need to take a flashlight or other lighting devices with them nor adjust the lighting.

%\subsubsection{Technology for the Low Vision Population.}
%Through interviewing with PVI and trainers, we noticed that despite people who were low vision often having different needs, few technology products mentioned during interviews were designed especially for people with low vision. In other words, most technology products were designed based on the blind population’s data and did not distinguish blindness from low vision. Consequently, low vision people's confidence level was lower than blind people. Thus, when designing technology devices, it would be important to take the low vision population’s needs into account. For example, for people with some residual vision, technology devices would be easier to use if they came with not only strong visual exteriors that had bright colors, lighting, and high contrast but also adjustable settings that allowed people with low vision to increase fonts, reverse contrast, and so on.

\subsubsection{Making Mainstream Kitchen Appliances Accessible.}
While various assistive technologies have been designed for PVI, we found it important to make mainstream technology accessible. In our study, even for low-tech tools, some PVI preferred mainstream options to specialized ones since the mainstream tools had better quality (e.g., Mary, Judy). This was probably because mainstream products had a significantly larger market and more competitors. The professionals also mentioned some clients did not want to use specialized technology since it may make them look different from others (Michael). Prior research has repeatedly shown that specialized technology may marginalize people with disabilities \cite{shinohara2011shadow, parette2004assistive, riemer1997factors}. Thus, designing accessible mainstream kitchen appliances is another important direction for future technology innovation. For example, similar to screen readers on computers and smartphones, the control interfaces of kitchen appliances should incorporate audio or tactile feedback for PVI to access.  

%the accessibility of mainstream technology is necessary. PVI relied on multiple sensory channels to extract information from the kitchen environment. We thus suggest incorporating multi-model feedback in kitchen technologies, especially the mainstream kitchen appliances. 
 
 %however, current  especially tactile and auditory cues. For tactile cues, most participants expressed complaints about how current technology and appliances often utilized flat screens. For example, many participants reported that induction stoves were challenging and sometimes unsafe to use because of their flat surfaces and the absence of dials and knobs, which made it hard for them to distinguish burner locations and adjust the heat. Therefore, for PVI to deal with flatscreens, it would be helpful to have tactile overlay attached to the surfaces with tactile or Braille labels on it to let PVI know each function and its position \cite{guo2017facade}. Additionally, when designing technology, tactile features should be incorporated so that PVI could use it more effectively. As for incorporating auditory cues, it would be helpful for each button to have a corresponding sound to distinguish different functions; for PVI who were using a technology device for the first time, it would be easier for their memory load and for them to learn if it had the option of reporting back or explaining the function of the button chosen by PVI to them. On top of that, when PVI were reading (e.g., recipes, food package information, etc.), the auditory feature would be helpful when combined with OCR technology, which would allow the device to read the detected text back to users \cite{fusco2014using, kostyra2017food}.

%\subsubsection{Remote Training through VR.}
%When it came to training, we proposed that remote training through VR devices could help PVI adapt to different kitchen setups. This was not only because COVID put some training on pause (e.g., small group training) but also because one of the biggest weaknesses of current training was its invariability where clients were trained in controlled environments and the training content might not be translated to their home kitchen. Thus, with VR devices, they allowed trainers to provide training in various settings as well as PVI to practice what they had learned in settings that resembled their home kitchen space.

\subsubsection{Trade-off between Automation and Agency.}
Our findings revealed the tension between automation and agency in technology design. On the one hand, some PVI (e.g., Hilary, Derek) indicated their desire for a smart kitchen that completes cooking tasks for them automatically. On the other hand, some professional trainers (e.g., Rachel, Maria) highlighted that advanced technology should not entirely replace PVI in their kitchen. They argued that PVI had emotional connections with the kitchen and wanted to cook “for the joy of it” (Maria). Future assistive technology should thus consider the tradeoff between automation and agency, assisting PVI to accomplish kitchen tasks independently and allowing them to enjoy cooking. 


%\subsection{Needs for follow-up training and mental support for AVI}
%guidelines:
%    1. all our AVI participants are trained but still they struggle
%    2. 

%\subsection{Reflection on Methodology.}
%The result of Study 1 shows the challenges and coping strategies related to cooking activities faced by blind participants and low vision participants and how they envisioned technology can help overcome the challenges in the future. Our findings in general resonate with prior works that explored cooking challenges of blind people. \cite{bilyk2009food, jones2019analysis, kashyap2020behaviors, li2021non}, 
%even though we had some findings that are quite different from some prior works, for example, we found gas stovetop is prefered over glass top or electric stovetops by blind participants, which is the opposite of what Li et al\cite{li2021non} had found. However, we reached opposite conclusion from two different perspectives (auditory feedback and ease of cleaning vs. ease of placement). This shows that cooking challenges and strategies are complicated in nature, and they need to be better understood by incorporating different angles through more studies in the future. 
%Moreover, instead of focusing on blind population, the majority of participants we recruited are low vision. They have adopted different strategies than blind participants since they can utilize their residual vision, for example, reading and interacting with appliances. By delving into the different cause of low vision people's cooking challenges, we can further design visual aid systems for them. 

%Enabled by contextual inquiry, our work complemented prior works with unique findings that are only available via observing and interviewing in participants' own kitchen space. First of all, we elicited in-situ challenges so as to better identify the gap between participants' coping strategies and reality. For example, participants kept things organized in the kitchen but still failed to keep track of things during cooking. 
%In addition, observation helps facilitate grounding process between researchers and participants, so that we can better interpret participants' action and words based on their own situation. For instance, some participants were so used to feeling around with hands and downplayed the safety risks through interview, which we can easily identify through observation. 
%Secondly, by observing cooking challenges and strategies across all the participants, we realized the constraints and generalizability of participants' strategies and adaptations depend on their cooking experience level, kitchen setup and dishes they cooked. For example, to tell doneness of food, a common strategy is to smell, however during one observation, we found the food might get overcooked when its smell is prominent enough to tell. Overall, contextual inquiry helps facilitate grounding process between researchers and participants, so that we can better interpret participants' action and words based on their own situation. Comparing the similarities and differences between prior works and ours, we realize cooking challenges and strategies of PVI are complicated in nature, and they need to be better understood by incorporating different angles  through more studies in the future. 

\subsection{Limitations and Future Directions.}
Our studies had limitations. First, due to the pandemic, we only observed 10 PVI and some were observed remotely via a video call, which could prevent us from observing some cooking details. In the future, we will recruit more participants and conduct all in-person studies to thoroughly observe participants during cooking. Second, we allowed the participants to autonomously choose a dish to cook. It was possible that they picked the dish that they were more familiar and comfortable with, which may limit the cooking challenges revealed in the observation. Future work should consider observing PVI in each specific cooking task to cover more comprehensive kitchen dynamics. 
Lastly, our exploration of rehabilitation training mainly focused on the professional's perspective. In the next step, we will focus on the visually impaired clients' perspectives and fully understand their training experiences and potential barriers they face. 

%the number of participants we recruited might not be enough to represent the PVI population and trainers population. For example, we only had one trainer with low vision while others were sighted, and it might be meaningful to gauge how trainers with visual impairments trained their clients differently than sighted trainers.  Future studies could include more diverse participants and have a more standardized design for observation (e.g., asking participants to cook similar dishes) in order to compare participants’ performance.

%Second, we connected and compared certain aspects in Study 1 with Study 2, participants we observed in Study 1 might tend to choose to cook dishes they were more familiar with, showing less difficulty performing activities than clients we observed and interviewed with in Study 2 might have.


%Lastly, we showed participants' diverse emotion and mentality during cooking which is a vital yet generally ignored factor that affect PVI's cooking experiences. Future research should explore how to support PVI's cooking mentally and possibilities to incorporate it into training sessions or assistive technology.

%From our study, we realized that participants with congenital visual impairment are more independent and confident about cooking than participants with acquired visual impairment because of the experience they gained throughout their lifetime. Rehabilitation training could be in place to catalyze this process. In order to make rehabilitation training more effective, we need to further understand the current gap between participants' situation and the training they can possibly get.


